Network-accelerated Active Messages

Remote Direct Memory Access (RDMA) improves host networking performance by eliminating software and server CPU involvement. However, RDMA has a limited set of operations, is difficult to program, and often requires multiple round trips to perform simple application operations. Programmable SmartNICs provide a different means to offload work from host CPUs to a NIC. This leaves applications with the complex choice of embedding logic as RPC handlers at servers, using RDMA's limited interface to access server structures via client-side logic, or running some logic on SmartNICs. The best choice varies between workloads and over time. To solve this dilemma, we present NAAM, network-accelerated active messages. NAAM applications specify small, portable eBPF functions associated with messages. Each message specifies what data it accesses using an RDMA-like interface. NAAM runs at various places in the network, including at clients, on server-attached SmartNICs, and server host CPU cores. Due to eBPF's portability, the code associated with a message can be run at any location. Hence, the NAAM runtime can dynamically steer any message to execute its associated logic wherever it makes the most sense. To demonstrate NAAM's flexibility, we built several applications, including the MICA hash table and lookups from a Cell-style B-tree. With an NVIDIA BlueField-2 SmartNIC and integrating its NIC-embedded switch, NAAM can run any of these operations on client, server, and NIC cores, shifting load in tens of milliseconds on server compute congestion. NAAM dynamically offloads up to 1.8 million MICA ops/s for YCSB-B and 750,000 Cell lookups/s from server CPUs. Finally, whereas iPipe, the state-of-the-art SmartNIC offload framework, only scales to 8 application offloads on BlueField-2, NAAM scales to hundreds of application offloads with minimal impact on tail latency due to eBPF's low overhead.

==> tex/background.tex <==
\begin{table*}[t]
\centering\renewcommand\cellalign{lc}
\setcellgapes{1pt}\makegapedcells
\footnotesize
\begin{tabular}{l|ccccl} 
    \toprule
    \textbf{System} & \textbf{\makecell{Programmability}} & \textbf{\makecell{Multi-Tenant\\Scaling}} & 
    \textbf{\makecell{Dynamic\\offloading}} & 
    \textbf{\makecell{Commodity\\SmartNIC}} & \textbf{Description}\\
    %\Xhline{2.5\arrayrulewidth}
    \midrule
    RMC~\cite{AmaroRMC2020}		        & \cmark & - 	  & \xmark & \cmark & Description     	\\
    PRISM~\cite{BrukePrism2021} 		& \xmark & ? 	  & \xmark & \cmark & Description     	\\
    StRoM~\cite{SidlerStorm2020} 		& ?		 & ?	 	  & \xmark	   & \xmark    & Description		\\
    1RMA~\cite{Singhvi1RMA2020} 		& 		 & 	 	  & 	   & 	    & Description	    \\
    Snap~\cite{snap} 					& \cmark & \cmark & N/A    & N/A    & Description 		\\
    iPipe~\cite{ipipe} 					& \cmark & \xmark & \cmark & =  	& Description       \\
    Bertha~\cite{bertha} 				& 		 & 	 	  & 	   & 	    & Description	    \\
    \textbf{NAAM}                   	& \cmark & \cmark & \cmark & \cmark & Description \\ \bottomrule
	%\Xhline{2.5\arrayrulewidth}
\end{tabular} 
\vspace{0.1in}
\caption{A comparison of existing RDMA approaches.} %Most of them are bounded to a specific target (i.e., Openflow, DPDK, RMT). Although NFReducer is not, it cannot optimize code based on input traffic profiling.}
\label{table:comparison}
\vspace{-0.2in}
\end{table*}

\section{Background and Motivation}
\label{sec:motivation}

Modern datacenter CPUs cannot keep up with the rapid growth of network bandwidth. Current NICs can handle 400 Gbps, while 800 Gbps is coming soon. However, the computing capacity of data center CPUs isn't increasing at the same rate. To solve this issue, remote direct memory access capable NICs emerged. It can access remote memory, bypassing the host CPU and offloading the networking stack to the server NIC. This reduces tail latency and increases throughput while using fewer server and client CPU cycles. For these advantages, modern data centers have started adopting RDMA for various distributed applications, including distributed machine learning, graph processing, key-value stores, etc. 
%\seb{You are already saying this in the intro.}
There are two sets of instructions for RDMA, one-sided and two-sided. These are called RDMA verbs. With one-sided RDMA verbs, remote memory can be accessed directly from the NIC without intervening the host CPU. However, it is limited in terms of programmability. It can only perform primitive memory read/write operations. To do more complicated operations e.g., walking a hash table, memory access logic needs to be written in the client, which requires multiple round trips for the operation with the primitive read/write ops and increases latency significantly. With two-sided RDMA verbs, memory access logic can be executed in the server. This reduces latency for complicated memory operations but consumes server CPU cycles. This leaves us with two different models for writing RDMA applications. The best model for a particular application depends on various factors, e.g., compute capacity, data access pattern, number of data-dependent operations, etc. Application developers have to carefully consider which model to use before deployment, which is a complex problem as all of these parameters vary depending on the workload and might change over time.

At the same time, smartNICs have emerged that can offload general purpose compute, and these introduce even more models for writing applications.
These smartNICs employ their own processing elements, memory, and non-volatile storage for persistence, and these smartNICs can offload arbitrary application logic entirely onto the smartNIC. This reduces the number of consumed CPU cycles on the main CPU. This can also improve application latency as the application is closer to the network. The processing element of a smartNIC can be either FPGA based or SoC based. The FPGA based smartNIC is mostly suitable for domain-specific tasks which have a relatively simple data structure. The SoC based smartNICs are more general in that sense, as they can offload any application logic with complex data structures. These smartNICs are often equipped with ASIC accelerators to accelerate domain-specific tasks, for example, TCP/UDP offload, regular expression matching, encryption/decryption, storage acceleration, etc. The SoC based smartNICs usually have multicore ARM/MIPS processors. Broadly, these SmartNICs can be divided into two categories on-path and off-path smartNICs. In case of on-path SmartNICs the processing elements sit in the data path. Every packet goes through the smartNIC processing cores.
For this reason, there is a contention for CPU resources for offloaded applications and packet processing. Usually, they can't run a full-fledged operating system. Low level interface is exposed to manipulate packets from the cores. They can be programmed using the SDK provided by the vendor. On the other hand in case of off-path smartNIC, the compute elements and the data path are divided by a hardware switch embedded in the smartNIC. The smartNIC can act as a separate endpoint, and flow rules can be installed in the hardware switch to steer packets either to the host cores or to the smartNIC cores. These types of smartNICs can run full-fledged operating systems like Linux with full networking stack or kernel-bypassed systems like DPDK. On these smartNICs, the application development process is the same as the host in that applications can be recompiled for the specific smartNIC architecture to execute in the smartNIC.  However, even with these NICs, application developers must still manually reimplement functions in multiple different ways to allow for computation to be moved between smartNIC cores and main CPU cores. Also, in our work, we focus on off-path smartNIC unless otherwise specified.

There have been several research works for offloading general compute to the smartNICs. The state-of-the-art offloading framework iPipe uses actor-based programming model for offloading tasks to smartNIC. Each actor executes a specific function. iPipe assumes a single queue abstraction for distributing packets to the NIC cores. This will not scale for off-path smartNICs. To provide single queue abstraction; few cores need to be dedicated just for this purpose, which will reduce NIC processing capacity significantly. To provide isolation for off-path smartNICs each actor will run as a separate thread/process. This model is suboptimal for modern multi-tenant datacenters where multiple applications from different tenants are co-located in the same platform. iPipe model can only scale functions up to the available CPU cores in the system. In the evaluation~\ref{sec:eval}, we will show how iPipe's performance quickly falls off as the number of functions increases.
%\seb{I believe this section lacks a strong motivation. It seems to be a blend of an introduction and an abstract. We should emphasize the key features that NAAM offers and highlight how existing works fall short in delivering these features.}

% StROM is implemented on FPGA. So, FPGA synthesis is needed to install functions. But the mentioned in the paper they can programmed high level C++. Should we call it programmable?

%\subsection{Existing Approaches}
%\label{subsec:existing-approaches}

%\subsubsection{RMA Frameworks}

%\afq{iPipe, Bertha, RMC, PRISM}

%{\color{red} Detailed paragraph exactly about why iPipe will fail to work to solve this... -- mention portability, but focus mainly on scaling mutually distrusting functions.}

%\subsubsection{SmartNIC Programming Frameworks}

%\begin{table}[t]
%\centering
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{c|cccc}
%\toprule
%System &
%  \begin{tabular}[c]{@{}c@{}}Programmability\end{tabular} &
%  \begin{tabular}[c]{@{}c@{}}Multi-Tenant\\ Scaling\end{tabular} &
%  \begin{tabular}[c]{@{}c@{}}Dynamic\\ Offloading\end{tabular} &
%  \begin{tabular}[c]{@{}c@{}}Commodity\\ SmartNIC\end{tabular} \\ \midrule
%RMC~\cite{AmaroRMC2020} & + & ? & - & + \\
%PRISM~\cite{BrukePrism2021} & - & ? & - & + \\
%StRoM~\cite{SidlerStorm2020} & & & & \\
%1RMA~\cite{Singhvi1RMA2020} & & & & \\
%Snap~\cite{snap} & + & + & N/A & N/A \\
%Floem~\cite{floem} & & & &\\
%iPipe~\cite{ipipe} & + & - & + & =\\
%Bertha~\cite{bertha} & & & &\\
%NAAM & + & + & + & + \\
%\bottomrule
%\end{tabular}
%}
%% \vspace{-0.3cm}
%%\scaption{A comparison of existing RDMA approaches.}
%
%%{\color{red} Need to add SmartNIC programming approaches in this table.}}
%\label{table:comparison}
%\end{table}

%\subsection{Design guidline}

%\noindent \textbf{Automatic placement of applications}
%\newline

%\afq{Motivate reader about the complexity of deciding the placement of applications
%in different locations based on the resource requirements.}
%Different workloads have different requirements for resources to run. For example, available compute, memory, PCIe bandwidth etc. Determining these requirements at the application development time is difficult or impossible in some cases. As the requirements might evolve over time. Based on the resource requirements, there are different choices for the application to run. It can be run on the server, on the client, or on the server attached smartNIC. Also, it is possible to run part of the function in one location and part of it in another location. Each of these different locations have different tradeoffs. For example, a linked list is memory heavy and accesses are dependent on each other, so it will be efficient to run them on the server or offload on the smartNIC. On the other hand, a hashtable is compute heavy. So, once can consider to run the hash computation on the client as they are stateless and key/value operations on the server. Considering all these choices even before deploying the application is a near-impossible task. NAAM can monitor all of these resources and decide policies on runtime based on that
%to run all or parts of the application in different locations, which optimizes throughput and latency. And if, in some situations, it’s not possible to optimize or a bad decision is taken, then NAAM realizes that and defaults back to running the application on the server host.
%\newline

%\begin{figure}[t]
%\includegraphics[width=\columnwidth]{figures/placement-motivation.png}
%\caption{Different kinds of resources in different axis
%and place application in the right place according to
%resource requirement to motivate the need for automatic application placement.}
%\end{figure}

%\noindent \textbf{Platform agnostic abstractions for RDMA}
%\newline

%RDMA applications are difficult to be developed. For example, the application
%programmer needs to register shared memory between NIC and the App ahead of
%time. Also, application logic includes a lot of RDMA communication logic, which
%is not desirable from the maintainability and debuggability standpoints.
%Moreover, deciding over 1-sided and 2-sided verbs requires a deep understanding
%of the infrastructure and has a critical implication on the applications’
%performance. Unfortunately, this information is usually hardly available at the
%development time, or taking all these factors into account can be cumbersome
%for the application developers.

%Further, CPU performance has already stagnated due to the end of Dennard
%scaling, and achieving higher performance seems to be impractical. NAAM is
%inspired by these observations and aims to provide a better abstraction by
%first providing higher flexibility to the programmer and allowing for running
%custom eBPF programs at the NIC, second, achieving higher performance by
%addressing problems associated with 1-sided, and 2-sided verbs via NIC acceleration.

%Figure X demostrates how RDMA works in a remote scenario. \as{I should have a
%figure and put numbers of describe things here.}

